Exploring the Landscape of Spatial Robustness

The study of adversarial robustness has so far largely focused on perturbations bound in p-norms. However, state-of-the-art models turn out to be also vulnerable to other, more natural classes of perturbations such as translations and rotations. In this work, we thoroughly investigate the vulnerability of neural network--based classifiers to rotations and translations. While data augmentation offers relatively small robustness, we use ideas from robust optimization and test-time input aggregation to significantly improve robustness. Finally we find that, in contrast to the p-norm case, first-order methods cannot reliably find worst-case perturbations. This highlights spatial robustness as a fundamentally different setting requiring additional study. Code available at https://github.com/MadryLab/adversarial_spatial and https://github.com/MadryLab/spatial-pytorch.

==> black_canvas.tex <==
\section{Black Canvas}
\input{figures/black_canvas_table}


==> figures/majority_table_small.tex <==
\begin{table}[!ht]
\caption{
Majority Defense.
Accuracy of different models on the natural evaluation set and against a combined rotation and translation adversary using aggregation of multiple random transformations. For each image, natural or perturbed, $10$ random transformations are performed and the model outputs a majority vote over predicted labels. For the full table, see Figure~\ref{tab:majority} of Appendix~\ref{app:omitted}.
}
\label{tab:majority_small}
\begin{center}
{\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4.1pt}
\begin{tabular}{c|ccc|ccc|ccc}
& \multicolumn{3}{c|}{MNIST} &\multicolumn{3}{c|}{CIFAR-10}&\multicolumn{3}{c}{ImageNet}\\ 
& Std. & Aug. & W-10 & Std. & Aug. & W-10 & Std. & Aug. & W-10\\
\hline 
Nat. Acc. & 99.31\% & \textbf{99.53}\% & 99.48\% & \textbf{92.62}\% & 90.02\% & 91.34\% & 75.96\% & 65.96\% & \textbf{76.14}\% \\
Nat. Vote & 98.71\% & \textbf{99.41}\% & 99.40\% & 80.37\% & 92.70\% & \textbf{93.38}\% & 73.19\% & 72.44\% & \textbf{74.92}\% \\
\hline
Grid Acc. & 26.02\% & 95.79\% & \textbf{97.32}\% & 2.82\% & 58.90\% & \textbf{69.17}\% & 31.42\% & 32.90\% & \textbf{52.76}\% \\
Grid Vote & 18.80\% & 95.32\% & \textbf{96.95}\% & 7.85\% & 69.65\% & \textbf{77.33}\% & 40.21\% & 44.46\% & \textbf{56.45}\% 
\end{tabular}
}
\end{center}
\end{table}

